Three-dimensional wave structures and their formation mechanisms in a non-premixed hydrogen-air rotating detonation combustor

Three-dimensional large-eddy simulations (LES) are performed for a non-premixed hydrogen-air rotating detonation combustor (RDC) and validated against experimental high-frequency pressure signals and OH* chemiluminescence features. Combined analysis of experimental snapshots and numerical results identifies the primary detonation wave (PDW), downstream oblique shock (DOS), detached detonation waves (DDWs), and inward-transmitted shock (ITS). Their three-dimensional structures and interactions are examined. Recirculation behind the backward-facing step (BFS) retains hot products near the inner wall, whereas fresh reactants occupy the outer-wall region. Discrete hydrogen jet columns (HJCs) are distributed within the fresh reactants. The PDW and its principal heat-release region propagate mainly through the outer fresh-mixture layer. Multiple DDWs successively separate from the upstream side of the PDW and propagate upstream along the HJCs. DDW evolution comprises detonation-front deformation, detonation-front separation, upstream propagation along the HJCs, heat-release decay and recovery near the injectors. DDW formation arises from competition between PDW-driven circumferential propagation and upstream propagation supported by the local fuel distribution. The DDWs generate diffracted shocks that influence the wave system. Pressure disturbances transmitted from the PDW into the hot-product layer form an ITS that leads the PDW in circumferential phase. The ITS exhibits reduced net heat release near its front and induces transmitted and reflected oblique shocks in the fresh-mixture layer. Periodic blast waves generated by DDW shock diffraction propagate inward and catch up with the ITS, producing pressure disturbances that may sustain its propagation. These findings connect experimental emission features to three-dimensional wave structures and clarify their formation and interaction.

==> submission_cleanup.tex <==
% Remove instructional placeholders supplied by the author-guide class.
% No changes to the original class, type sizes, margins or body spacing.
\makeatletter
\patchcmd{\ps@titlepage}{\hbox to \textwidth{{\fboxsep0pt\fbox{\parbox{\textwidth}{\par\vskip2.7pc\centerline{Banner appropriate to article type will appear here in typeset article}\par\vskip2.7pc}}}}}{}{}{}
\patchcmd{\ps@titlepage}{\hbox to \textwidth{{\fboxsep0pt\fbox{\parbox{\textwidth}{\par\vskip2.7pc\centerline{Banner appropriate to article type will appear here in typeset article}\par\vskip2.7pc}}}}}{}{}{}
\patchcmd{\@maketitle}{(Received xx; revised xx; accepted xx)}{}{}{}
% Preserve the template's volume/article/page numbering; remove only guide banners.
\def\submissionpagenumber{\cppagefont\thepage}
\def\oddabsfooterflag{\hbox to\textwidth{\hfill{\submissionpagenumber}}}
\def\evenabsfooterflag{\hbox to\textwidth{{\submissionpagenumber}\hfill}}
\def\pagelimitfooter{\hbox to\textwidth{{\submissionpagenumber}\hfill}}
\makeatother

